Functional Split of In-Network Deep Learning for 6G: A Feasibility Study

In existing mobile network systems, the data plane (DP) is mainly considered a pipeline consisting of network elements end-to-end forwarding user data traffics. With the rapid maturity of programmable network devices, however, mobile network infrastructure mutates towards a programmable computing platform. Therefore, such a programmable DP can provide in-network computing capability for many application services. In this paper, we target to enhance the data plane with in-network deep learning (DL) capability. However, in-network intelligence can be a significant load for network devices. Then, the paradigm of the functional split is applied so that the deep neural network (DNN) is decomposed into sub-elements of the data plane for making machine learning inference jobs more efficient. As a proof-of-concept, we take a Blind Source Separation (BSS) problem as an example to exhibit the benefits of such an approach. We implement the proposed enhancement in a full-stack emulator and we provide a quantitative evaluation with professional datasets. As an initial trial, our study provides insightful guidelines for the design of the future mobile network system, employing in-network intelligence (e.g., 6G).

==> sections/backup_jiahe/abstract.tex <==
Abstract goes here

==> sections/backup_jiahe/acknowledgement.tex <==
\section*{Acknowledgment}
This work has been partially funded by the Federal Ministry of Education and Research (Germany) under the funding code 01IS17044, and partially funded by the German Research Foundation (DFG, Deutsche Forschungsgemeinschaft) as part of Germany’s Excellence Strategy – EXC 2050/1 – Project ID 390696704 – Cluster of Excellence “Centre for Tactile Internet with Human-in-the-Loop” (CeTI) of Technische Universität Dresden.
Responsibility for the content of this publication lies with the authors.

==> sections/backup_jiahe/background.tex <==
\section{Background}\label{sec:background}

\subsection{Related work}\label{subsec:related_work}
BSS is a fundamental data pre-processing technology for many applications, e.g., audio analysis, natural language processing, speech recognition, MIMO, etc..
Popular ways to solve a \ac{bss} problem are machine learning-based \ac{ica} methods~\cite{Hyvarinen1999Fastrobustfixed, Wu2021NetworkProcessingAcoustic, Wu2021ComputingMeetsNetwork} and neural network-based methods~\cite{Luo2019ConvtasnetSurpassing, Stoller2018WaveUNet}. However, the neural network-based methods have a significant advantage over the ICA methods in terms of data volume. The ICA methods are a determined system, where the input data must be the same number of data sets as the number of sources, while the neural network-based methods are an underdetermined system, independent of the number of sources, which requires only one set of input data.
Therefore, in IoT networks, the neural network-based methods can effectively reduce the stress on network bandwidth and data transmission time by greatly reducing the size of the transmitted data.

The field of the BSS has been revolutionized thanks to deep learning techniques.
In contrast to ICA, deep learning-based models involve only a forward inference process after the training procedure.
The deep learning-based approach can generate separated source signals with a fixed output sequence as outputs.

Most previous audio separation methods have been developed in the time-frequency (T-F, or spectrogram) representation of the given mixed signal. 
The time-frequency (T-F, or spectrogram) representation of the mixed-signal, is estimated using the short-time Fourier transform (STFT).
Its objective is to estimate the clean source signal from the mixed time-frequency signal.
However, the T-F-based approach has the following drawbacks that affect the quality of separation and service latency.
First, STFT is a generic signal transformation that may not the best choice for  BSS-problem. The STFT transformation loses some time-domain information and introduces an upper limit to the quality of the separation.
Second, the high precision separation from the T-F representation requires a high-resolution frequency decomposition of the mixed-signal, which demands a long time window to perform the STFT computation as well.
It can significantly increase the additional service latency.

To overcome the above shortcomings, recent studies have proposed separation methods based on time-domain signals.
Most time-domain-based systems rely heavily on the masking separation strategy proposed by Conv-TasNet\cite{Luo2019ConvtasnetSurpassing}.
It utilizes parameter-learnable convolutional layers instead of STFT transformation to outperform the T-F representation-based methods.
Also, it uses a lightweight model to ensure low computational complexity latency.


\subsection{Challenges}\label{subsec:challenges}
Due to the massive parameters of deep neural networks, it usually needs to occupy the main computational resources on the server-side.
And offloading the deep neural network computation process to the network can effectively free up the computational resources on the server-side.
In practical deployment and inference, most deep neural networks use a straightforward computational structure, i.e., each neural network layer needs to be computed only once.
Intuitively, offloading computational processes to the network requires splitting and deploying different parts of the NN model in different VNFs.
However, the following challenges usually need to be addressed to accomplish this goal.
\begin{enumerate}
    \item Limited computing resources: Typically, VNF devices have limited computing resources. It cannot run all the computational processes like the server side.
    Therefore, when deploying computational processes in VNF, it is necessary to consider whether the deployed computational processes and resources match. Also, when there are multiple VNFs, the computing resources of each VNF should be utilized as evenly as possible.
    \item Additional cache time: When a deep learning model performs inference, the computational process of most layers requires the entire output of the previous layer as input.
    Compared to centralized deployments, VNFs require additional storage time to receive the data required for computation.
    Therefore, the deployment needs to be designed in a way to offset the impact of the extra storage time on the service latency.
    
\end{enumerate}


==> sections/backup_jiahe/bio.tex <==
\vskip 0pt plus -1fil
\begin{IEEEbiographynophoto}
{Jia He} (jia.he@mailbox.tu-dresden.de) is a graduate student with the Deutsche Telekom Chair of Communication Networks at Technische Universität Dresden (TU Dresden), Germany, since 2017.
He received his Bachelor of Science degree from Xidian University, China, in 2015.
His interests during his studies are data analysis in networks.
\end{IEEEbiographynophoto}

\vskip -2\baselineskip plus -1fil
\begin{IEEEbiographynophoto}
{Huanzhuo Wu} (huanzhuo.wu@tu-dresden.de) is a research fellow with the Deutsche Telekom Chair of Communication Networks at Technische Universität Dresden (TU Dresden), Germany.
He received his M. Sc. degree in Computer Science at TU Dresden, in 2016.
His research interest is data analysis on Blind Source Separation and in-network computing.
\end{IEEEbiographynophoto}

\vskip -2\baselineskip plus -1fil
\begin{IEEEbiographynophoto}
{Xun Xiao} (xun.xiao@huawei.com) ***.
\end{IEEEbiographynophoto}

\vskip -2\baselineskip plus -1fil
\begin{IEEEbiographynophoto}
{Riccardo Bassoli} (riccardo.Bassoli@tu-dresden.de) is a senior researcher with the Deutsche Telekom Chair of Communication Networks at Technische Universität Dresden (TU Dresden), Germany. He received his B.Sc. and M.Sc. degrees in Telecommunications Engineering from the University of Modena and Reggio Emilia (Italy) in 2008 and 2010 respectively. Next, he received his Ph.D. degree from 5G Innovation Centre (5GIC) at the University of Surrey (UK), in 2016.
\end{IEEEbiographynophoto}

\vskip -2\baselineskip plus -1fil
\begin{IEEEbiographynophoto}
{Artur Hecker} (artur.hecker@huawei.com) ***.
\end{IEEEbiographynophoto}

\vskip -2\baselineskip plus -1fil
\begin{IEEEbiographynophoto}
{Frank H. P. Fitzek} (frank.fitzek@tu-dresden.de) is a professor and head of the Deutsche Telekom Chair of Communication Networks at TU Dresden, Germany.
He received his Dipl.-Ing. degree in electrical engineering from the Aachen University of Technology RWTH, Germany, in 1997 and his Dr.-Ing. degree in electrical engineering from Technical University Berlin.
\end{IEEEbiographynophoto}

==> sections/backup_jiahe/conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}



\add{Call for paper: \url{https://www.comsoc.org/publications/magazines/ieee-wireless-communications/cfp/ai-open-programmable-virtualized-networks}.
	Submission guideline:
	\begin{itemize}
		\item Articles should not exceed 4500 words (Introduction through Conclusions, excluding figures, tables and captions).
		\item Figures and tables should be limited to a combined total of six.
		\item Mathematical equations should not be used.
		\item A limit of 15 archival references is recommended. 
	\end{itemize}
	\url{https://www.comsoc.org/publications/magazines/ieee-wireless-communications/paper-submission}}

==> sections/backup_jiahe/evaluation.tex <==
\section{Evaluation}\label{sec:evaluation}

\subsection{Experimental setups}

\subsubsection{Scenarios}\label{subsec:evaluation_scenarios}
We conducted the evaluation on the network emulator, \ac{comnetsemu}~\cite{XiangOpenSourceTestbed}.
The unique advantage of \ac{comnetsemu} is its capability to provide functionalities of both \ac{nfv} and \ac{sdn}.
It allows for prototyping quickly COIN applications virtually of any scale.
As illustrated in~\cref{fig:conv_tasnet_arch}, we set up a multi-hop topology with switches as intermediate network nodes. Each switch can perform either or both operations of forwarding and data processing.
A client connects to the network and sends the observed mixtures using \ac{udp} traffic to the server.
All topology links have the same homogeneous bandwidth of $1$\,\textit{Gbps} and a fixed propagation delay of $10$\,\textit{ms}.
These specifications are typical for the devices in the network.
The purpose is to examine the benefits of in-network computing without superior specifications of high-end infrastructure.
We also assume that all devices and connections are general-purpose and available as commercial-off-the-shelf.

We also use FastICA, which is a machine learning-based BSS method, as a baseline system to compare with the artificial intelligent-based Conv-TasNet. Meantime, the in-network computing variant of FastICA, pICA, is used, to compare with the in-network computing Conv-TasNet. \hwcmt{The description of reference systems will be extended. Name for each reference system is needed for later discussion and legend in the figures.}

We implement the client and server functions in Python.
For each configuration of a parameter set, we performed 50 measurements in which the client sends the mixture matrix to the server.
We calculated the median results together with their 95\% confidence intervals. 
Each network node forwards packets to the server at the fastest possible speed.
When operating with in-network computing, the \ac{sdn} controller inserts rules into the flow table of each router to forward the data traffic through each network node to build an \ac{sfc}.

All emulations were done on a \ac{cots} server with an Intel(R) Xeon(R) Gold 6148 CPU @ 2.40GHz and 4GB RAM using Ubuntu 18.04.4 LTS.

\subsubsection{Metrics}\label{subsec:evaluation_metrics}
To assess the \ac{qos} of the Conv-TasNet service, we introduce the metric, which is the \textit{service time} observed at the client.
The metric measures the time difference between a request message sent by the client and its respective response from the server received at the client.
The service time includes transmission, cache, and computing time introduced by network nodes and the server.
The metric directly addresses the concern about the overhead introduced by offloading the computing among network nodes.
Together with the computing time, the service time allows us to assess both the benefit and cost of in-network computing collectively.

To measure the computing load at the server, we introduce the \textit{residual computing time} metric.
It is the duration that the server needs to compute until the source separation completes.
A small residual computing time means that the network nodes already offload a large portion of the computing. Thus, the remaining computing load is small.
On the contrary, a significant computing latency means that the server still needs to compute a large portion of the workload.

\subsubsection{Dataset}\label{subsec:evaluation_dataset}
We pick a published open dataset from~\cite{Purohit_DCASE2019_01}, called Malfunctioning Industrial Machine Investigation and Inspection (MIMII). 
The main reasons for choosing the MIMII dataset are as follows.
First, it is a well-known dataset that is widely referenced in research and engineering for acoustic machine anomaly detection.
In addition, it exactly reflects the theme of this work, i.e., processing the most relevant acoustic data of factory machines from industry rather than random acoustic data such as music or daily life data.
This dataset has collected $26092$ normal and anomalous operating sound data of four types of machines (i.e., valves, pumps, fans, and slide rails). $8$-second-long audio of each segment is used, which is single-channel with a sample rate of $16$kHz. The size of one data source is $128k$ (i.e., sample rate$\times$duration).
A mixing matrix will be applied to noise, simulating mutual interference before being received by \ac{iiot} sensors. At the client, the input data is received.

\subsection{Service time}

\begin{figure}[t]
	\centerline{\includegraphics[width=\columnwidth]{figures/service_latency_boxplot.pdf}}
	\caption{Total service time.}
	\label{fig:service_latency_boxplot}
\end{figure}

\cref{fig:service_latency_boxplot} shows the service times of the experimental candidates under different network scales.
First, it is found that the service time of the AI-based Conv-TasNet is much lower than that of the traditional ICA algorithm. The reduction in service time of the AI approach is mainly due to the fact that this algorithm requires less input data volume than the ICA algorithm, which in turn has a huge advantage in transmission delay.
Secondly, the stability of Conv-TasNet is also much better than that of ICA algorithm, which can be observed by the height of the boxplots and the position of the quartiles. The main reason for this observation is that the Newton optimization of the traditional ICA algorithm is closely related to the characteristics of the input data, and the number of optimization steps may fluctuate. In contrast, the artificial intelligence method is related to the scale of the neural network as well as the data volume in the inference stage, independent of the characteristics of the input data.
Based on these two points, we believe that the AI-based Conv-TasNet method has a huge advantage in terms of the transmitted data volume and computational stability when solving the same BSS problem.

From~\cref{fig:service_latency_boxplot}, one can find a drawback of in-network Conv-TasNet.
For traditional ICA algorithms, pICA often outperforms the centralized FastICA. This advantage comes from the fact that in-network computing processes the data while it is being transmitted, which reduces the workload on the server and thus the overall service time.
However, in-network Conv-TasNet does not outperform centralized Conv-TasNet in terms of service time. Instead, the gap becomes larger as the available network computing resources increase, i.e., the number of switches increases.
In particular, when there are 5 switches in the network, the service time of in-network Conv-TasNet is even slightly higher than that of pICA, which is almost the same as FastICA.
This observation suggests that although the Conv-TasNet has offloaded partial computational tasks from the server to the network, this offloading does not result in a reduction in service time. In the next section, we will investigate the reasons for this observation in detail.

\subsection{Time consumption analysis}

\begin{figure}[t]
	\centerline{\includegraphics[width=\columnwidth]{figures/all_time_bar.pdf}}
	\caption{Time consumption. \hwcmt{Need to be optimized.}}
	\label{fig:all_time_bar}
\end{figure}

% \begin{table}[t!]
%     \def\arraystretch{1.5}
%     \centering
%     \caption{Time consumption comparisons.}
%     \label{tab:evaluation_time}
%     \begin{tabular}{L{2cm}|C{1.2cm}|C{1.2cm}|C{1.2cm}|C{1.2cm}}
%     \toprule[1pt]
%     \bf Median Time & \bf \bf INC Conv & \bf Conv & \bf pICA & \bf FastICA \\
%     \midrule[0.5pt]
%     \emph{Service Time} & 0.925 & 123.61~ms & 3.63M & 0.42G \\
%     \hline
%     \emph{Forwarding Time} & 0.764 & 87.08~ms & 3.20M & 0.35G \\
%     \hline
%     \emph{Computing Time} & 0.760 & 165.65~ms & 11.02M & 4.37G \\
%     \hline
%     \emph{Cache Time} & 0.895 & 254.23~ms & 19.22M & 9.08G \\
%     \bottomrule[1pt]
%     \end{tabular}
% \end{table}

\cref{fig:all_time_bar} details the median time spent on each step of solving the BSS problem using Conv-TasNet for both in-network and centralized scenarios: computing time, transmit time, caching time, and overall service time.

By analyzing the service time and each individual time consumed, i.e., compute time, transmit time, and cache time, shown in~\cref{fig:all_time_bar}, it is shown that in-network Conv-TasNet has the advantage of reducing the time by overlapping data processing and data transmission.
The service time of in-network Conv-TasNet is between $885.92~ms$ and $2465.06~ms$.
However, the sum of transfer, computation, and cache time is between $1233.49~ms$ and $3948.62~ms$.
The overlap time of in-network Conv-TasNet is between $28.18\%$ and $37.57\%$.
As the number of network devices involved in computing increases from 1 to 5, this overlap grows.
Compared with the centralized Conv-TasNet, its overlap is 0.
The reason for this result is that by deploying part of the data processing logic of Conv-TasNet as a network function on the network device in the transmission path through the network softwarization technologies, the data processing tasks that were originally centralized on the server are offloaded to the network.
This part of the offloaded data processing occurs simultaneously with the data transmission, which leads to overlapping time consumption.

However, in-network computing incurs other additional overheads, leading to the observation that the overall service time of the in-network Conv-TasNet is higher than that of the centralized Conv-TasNet, leaving more critical issues to be addressed in this area.

Comparing the time consumption of the two scenarios, it is obvious that the computing time is basically the same: $115.17~ms$ to $191.31~ms$.
This is because the total amount of computing tasks is the same, and each network device performing the computing task has the same computing power in the given network setup, so the computation time is the same.
Therefore, the difference in the total service time between in-network and centralized computing is mainly due to the difference in transmit time and cache time.

Since the first step of the Conv-TasNet operations is the encoder, this step results in an expansion of the data volume. 
The encoder of the in-network Conv-TasNet is executed early stage, thus, the amount of data transferred is extended compared to the centralized Conv-TasNet where only non-encoded data is transferred.
Such data volume expansion leads to an increase in the transmission time.
However, this increase is only due to the first encoder step and is not related to the number of switches involved in the subsequent computation. 
Therefore, in our measurement results, the transmission time of in-network Conv-TasNet stays within $751.96~ms$ to $856.18~ms$, taking into account the propagation delay.
The transmission time of the centralized Conv-TasNet lays in the range of $324.42~ms$ to $484.88~ms$.

The most noticeable aspect of~\cref{fig:all_time_bar} is the cache time of the in-network Conv-TasNet. 
Its cache time increases gradually with the number of network devices involved in the computation. 
In our measurements, when the number of network devices involved in the computation increases from 1, through 3, to 5, the caching time also enlarges from $304.58~ms$, through $1519.16~ms$, to $2972.12~ms$, which raises up from $14.37\%$ to $64.43\%$.
In contrast, for the centralized Conv-TasNet, since the intermediate network devices do not need to perform computation, they do not need to cache data, so its caching time is only $0.69~ms$ at most.
In particular, this cache time occurs only for the in-network Conv-TasNet, because each network device participating in the computation needs to cache enough data to execute the AI logic as a network function. 
As the number of network devices involved in the computation gradually increases, this cache operation is executed more frequently.
This increase significantly impairs the overall service time of the in-network Conv-TasNet.
\hwcmt{Maybe one more figure/table to show the correlation of data volume/cached packet number and cache time.}

\subsection{Challenge and outlook}
Overall, the additional time overhead of in-network Conv-TasNet due to data volume expansion for each of the three network settings is:
\begin{itemize}
    \item 1 switch: $20.17\%$ more transmission time and $14.37\%$ more cache time, in total $34.54\%$;
    \item 3 switches: $9.10\%$ more transmission time and $37.25\%$ more cache time, in total $46.35\%$;
    \item 5 switches: $5.79\%$ more transmission time and $64.43\%$ more cache time, in total $70.22\%$.
\end{itemize}
The time savings of in-network Conv-TasNet by overlap are:
\begin{itemize}
    \item 1 switch: $28.18\%$;
    \item 3 switches: $30.79\%$;
    \item 5 switches: $37.57\%$.
\end{itemize}

It can be seen that although in-network computing reduces part of the overall service time by overlaying the data transfer and data processing parts, the data volume expansion is caused by the common operations of convolutional neural networks, i.e., high-dimensional mapping, results in a huge increase in transmission and caching time.
We believe that deploying CNNs for in-network computing still has great potential to reduce service latency, however, the primary problem that needs to be addressed in the future is eliminating data volume expansion.

On the one hand, this problem can be solved by designing proprietary CNN structures, such as IA-Net-Lite~\cite{Wu21:InNetworkProcessingLowLatency}, to perform traffic filtering to address the problem of data bloat. The drawback of this approach is that it is not a general-purpose solution, and each CNN needs to be designed with respect to its purpose.
On the other hand, data volume expansion may be tackled from a network design perspective, e.g., through transmission data compression, or multi-path concurrency.

==> sections/backup_jiahe/introduction.tex <==
\section{Introduction}\label{sec:introduction}



\xxcmt{I searched some papers and try to purify our idea. There are some work about using NN to do inference for sure (e.g., do classification and so on). Therefore, we cannot just claim that ours is about cutting NNs into network devices and study its challenges.}

\xxcmt{We should go one level down, to say: we study BSS problem solved with NNs with COIN concept. Under this line, we clarify: 1. why BSS problem is different from other types of problems that are solved with using NNs, in order to show the uniqueness of our studied problem; 2. How BSS problem is solved with NNs in the literature, what are considered and what are not, to show our novelty and contributions; 3. For those not considered challenges/problems/potential issues, what's our opinions> why they are important. With this general logic flow, I think the whole idea should hold.}

\xxcmt{With the SotA, then in the following sections, we can start to introduce the method cutting NNs into networks with well justifications. After that, we start to introduce its opponent--pICA. Once this is done, we can go into the evaluation settings and results. At the end, we should put extensive and intensive discussions on the yielded observations; then we give our takeaway messages.}




\xxcmt{Only 15 references are allowed? I included the following papers:} \cite{Sapio2017NetworkComputationisa,Sanvito2018Cannetworkbe,Zhang2019DeepLearningMobile,Dutta2020DiscrepancyTheoreticalAnalysis,XiangOpenSourceTestbed,Liang2020edgebaseddeep,Xu2021GRACECompressedCommunication,Xavier2021ProgrammableSwitchesNetworking,Wu2021AbstractionbasedMulti,Wu2021NetworkProcessingAcoustic,Saquetti2021NetworkIntelligenceRunning,Wu2021ComputingMeetsNetwork,Yuan2022UnlockingPowerInline}

\hwcmt{Currently, the number of references is more than 15, we will remove some of them after all text is fixed.}

==> sections/backup_jiahe/method.tex <==
\section{Method}\label{sec:method}
\subsection{Introduction of Conv-Tasnet}
Conv-TasNet is an end-to-end time-domain speech separation method based on convolutional neural networks (CNN).
In Conv-TasNet,  the mixed mono waveform is patterned with a fully convolutional encoder-decoder model, which consists of three main components, namely encoder, separation, and decoder.

Encoder, as a collection of filters, maps the input time-domain signal data into a high-dimensional feature space $E$.
Meanwhile, this part of the data is reconstructed in the decoder to derive the separated signal, as shown in \cref{fig:conv_tasnet_arch}.

The separation part, as the main part of the model parameters, occupies most of the computational resources.
Its role is to extract the mask $M$ corresponding to each source to be separated from the encoder output $E$.
It is a stack of several 1D convolutional blocks with the same structure.
At the end of the separation process, an individual 1D-convolutional layer is attached to generate the mask according to the number of sources.

The decoder is designed to restore each individual source.
In the decoder operation, the high-dimensional feature data corresponding to each source is first obtained by the dot product of mask $M $and encoder data $E$.
After that, a 1D deconvolution layer is simply used to map the data from the feature space back to the time domain.
\begin{figure*}[t]
	\centerline{\includegraphics[width=\textwidth]{figures/conv-tasnet_new.pdf}}
	\caption{The architecture of Conv-TasNet and the corresponding network settings. Depending on the number of VNFs, the computational process is offloaded into the vnf network in different ways. Data transfer and computation are processed in parallel as much as possible, and data generated by the encoder is forwarded to the server in parallel while VNFs are computing to reduce service latency. In the figure, the green part represents the data generated by the encoder (VNF1 according to our setting), and the red part the data generated during the calculation of other VNFs. The data generated by the encoder is directly transmitted to the server-side. The server-side can receive the encoder data before receiving the VNF data. \hwcmt{The deployment method and time analysis could be divided into two figures, which are described and discussed separately.}}
	\label{fig:conv_tasnet_arch}
\end{figure*}
\subsection{Deployment}
To satisfy the three principles proposed above, we divide the model in the following way.
For a generic neural network model, the following analysis process is required to be performed when offloading to the network.

\begin{enumerate}
    \item Average arithmetic power: To maximize the use of the network's VNF devices, it is often necessary to split the model as evenly as possible.
    \item Local optimal data traffic: Deep neural networks transform raw data into high-dimensional feature representations by convolution or other operations. This process is usually accompanied by a variation in the scale of the data. To ensure that the transmission time after splitting is minimized, it is usually necessary to analyze the data traffic when splitting the model and split it in the locally optimal part if possible. This process sometimes conflicts with the first principle and requires appropriate trade-offs.
    \item Parallelization of computation and transmission: For VNFs with deployed sub-models, at computation time, each VNF is required to wait for all the computation results of the previous VNF, called cache time. As the number of VNFs increases, the storage time naturally increases. To reduce this additional time overhead, it is necessary to parallelize computation and transmission when deploying and transmitting data, i.e., perform computation while transmitting data that is unrelated to this VNF computation.
\end{enumerate}

First, to ensure that the computational resources of each VNF can be fully utilized, the number of parameters and computational complexity of the model's different layers need to be analyzed. It is guaranteed that the sub-models do not exceed the computational capacity limitation of the VNF after deployment.
Second, when considering the division place, it is necessary to analyze the data flow and the scale of the data in different parts of the model.
Normally, the data flow direction of the model is straightforward.
Therefore, only a single-link network structure needs to be considered when setting up the VNF.


Following the instructions of Conv-TasNet, we set up four blocks in the separation section, which have fixed sizes of input and output and the output data volume is relatively minimal.
Meanwhile, the encoder is always placed in the first vnf to receive the raw data, and the decoder is always deployed in the server to get the final result.
Since the final convolutional layer in the separation part exponentially scales up the data volume depending on the number of sources.
To save service latency it is merged with the decoder into one part.

\hwcmt{Generalising the description of deployments, rather than limiting it to specific 1, 3, and 5 VNFs.}
When the number of VNFs grows, it represents a gradual enrichment of computing resources within the network.
In order to simulate the deployment characteristics of the model with different computing resources, we set three cases with $VNF=1,3,5$.

\begin{enumerate}
    \item $VNF=1$: In this case, the separation part cannot be fully deployed in the VNF considering the limited network computing resources.
    Therefore, we evenly split the model and deploy the encoder and the first two blocks of the separation part in the unique VNF.
    In order to ensure the parallelization of computation and transmission, the data $E$ obtained after encoder computation is sent directly to the server-side, while the VNF continues to compute the mask data $M$ using $E$.
    On the server side, when the collection of the mask data $M$ is finished, the collected data is forwarded to the other two separate modules to derive the final mask $M$.
    \item $VNF=3$: In this setup, there are enough computing resources to allocate all the separation blocks.
    We deploy the four blocks equally in the last two VNFs while the encoder is deployed in the first VNF and the decoder is deployed on the server.
   The output $E$ from the encoder is sent to the second VNF, but also directly to the server.
   After receiving $E$ from VNF1 and $M$ from the last VNF, the server-side can directly calculate the final separation result.
   \item $VNF=5$: Similar to the case of VNF=3, the four blocks are equally allocated to the four VNFs.
\end{enumerate}

It is worth noting that as the number of VNFs increases, the distribution of models becomes increasingly "sparse".
Since the results of each layer of the neural network must use all the data of the previous layer, it leads to a gradual increase in the cache time of each VNF.

\subsection{AI as network functions}

==> sections/backup_xunxiao/background.tex <==
\section{Background}\label{sec:background}

\subsection{Related work}\label{subsec:related_work}
BSS is a fundamental data pre-processing technology for many applications, e.g., audio analysis, natural language processing, speech recognition, MIMO, etc..
Popular ways to solve a \ac{bss} problem are machine learning-based \ac{ica} methods~\cite{Hyvarinen1999Fastrobustfixed, Wu2021NetworkProcessingAcoustic, Wu2021ComputingMeetsNetwork} and neural network-based methods~\cite{Luo2019ConvtasnetSurpassing, Stoller2018WaveUNet}. However, the neural network-based methods have a significant advantage over the ICA methods in terms of data volume. The ICA methods are a determined system, where the input data must be the same number of data sets as the number of sources, while the neural network-based methods are an underdetermined system, independent of the number of sources, which requires only one set of input data.
Therefore, in IoT networks, the neural network-based methods can effectively reduce the stress on network bandwidth and data transmission time by greatly reducing the size of the transmitted data.

The field of the BSS has been revolutionized thanks to deep learning techniques.
In contrast to ICA, deep learning-based models involve only a forward inference process after the training procedure.
The deep learning-based approach can generate separated source signals with a fixed output sequence as outputs.

Most previous audio separation methods have been developed in the time-frequency (T-F, or spectrogram) representation of the given mixed signal. 
The time-frequency (T-F, or spectrogram) representation of the mixed-signal, is estimated using the short-time Fourier transform (STFT).
Its objective is to estimate the clean source signal from the mixed time-frequency signal.
However, the T-F-based approach has the following drawbacks that affect the quality of separation and service latency.
First, STFT is a generic signal transformation that may not the best choice for  BSS-problem. The STFT transformation loses some time-domain information and introduces an upper limit to the quality of the separation.
Second, the high precision separation from the T-F representation requires a high-resolution frequency decomposition of the mixed-signal, which demands a long time window to perform the STFT computation as well.
It can significantly increase the additional service latency.

To overcome the above shortcomings, recent studies have proposed separation methods based on time-domain signals.
Most time-domain-based systems rely heavily on the masking separation strategy proposed by Conv-TasNet\cite{Luo2019ConvtasnetSurpassing}.
It utilizes parameter-learnable convolutional layers instead of STFT transformation to outperform the T-F representation-based methods.
Also, it uses a lightweight model to ensure low computational complexity latency.


==> sections/backup_xunxiao/data_plane.tex <==
% 这个可能需要新增，因为本文主要提出的就是“我们做了一个这样的enhancement”
% 大体内容就是介绍一下系统架构，类似我们IoT-J那个，
% 然后说要在上面切DNN上去，有什么限制，挑战等等，
% 已经我们简单地principles

\section{In-network \ac{dl} enhancement for 6G}\label{sec:data_plane_enhancement}

\hwcmt{No touch on this section for HW and JH, only XX can edit this section.}

\xxcmt{I will add a pic here ...}

\subsection{DP \ac{dl} capability extension}
\xxtext{According to the reference architecture defined by 3GPP SA2, in core network part, DP mainly consists of \acp{upf} transporting \ac{pdu} sessions. A \ac{pdu} session represents a \ac{qos}-guaranteed connection between a UE and a \ac{dn} locating at edge or in a data center. As mentioned, in existing mobile network systems, \ac{upf} acts as a pure networking element, only transmitting bits and bytes in terms of the IP header of a data packet. In order to extend \ac{upf} with \ac{dl} capability, it is equivalent to enhancing \ac{upf} with a local \ac{dnn} component, which can be configured according to specific \ac{ml} applications.}

%The key reason is because the size of a \ac{dnn} is several magnitudes larger than the available resource on a \ac{upf}. Even if accommodating a whole \ac{dnn} is possible in the sense of storage, computationally operating it is also hard for the compute capability.
%\subsection{System model}\label{subsec:system_model}
%\begin{figure}[t!]
%	\centerline{\includegraphics[width=\columnwidth]{figures/network_topology.pdf}}
%	\caption{A network system architecture for in-network deep learning.}
%	\label{fig:network_topology}
%\end{figure}
%
%We consider a network system, as shown in~\cref{fig:network_topology}. This system consists of an ``access point'' (AP) node connected to a ``remote agent'' (RA) node in the cloud via an intermediate multi-hop forwarding path.
%Specifically, the collected data is aggregated at the AP node, which represents a WiFi AP or a cellular base station of a (non-public) network.
%The forwarding path between the AP node and the RA node can be determined dynamically according to the routing protocol or can be configured statically.
%The intermediate nodes of the forwarding path are programmable network devices that \acp{nf} can be assigned on.
%
%A \ac{dnn} consists of several neuron blocks, which can be single neurons, convolutional layers, fully connected layers, or other neural network elements.
%These neuron blocks are interconnected by neuron links.
%The input data of the \ac{dnn} is processed to give the output data required by the end user.
%The neuron blocks of a deep learning model can be deployed on these network nodes and RA nodes as \acp{vnf}.
%
%
%Before we start the further discussion, the following assumptions are made on the system setup:
%\begin{itemize}
%    \item The network topology is linear, and the number of intermediate nodes can be varied. Each intermediate node has limited computational power. Our research interest is to observe the behavior changing of in-network deep learning in the most fundamental linear network.
%    \item The packets forwarding and flow-table updating are automatically taken care of by the \ac{sdn} controller at the CP in the network, which is stable without transmission and connection failures. Our research focuses on enhancing the DP for in-network deep learning.
%\end{itemize}

\subsubsection{Challenges}\label{subsubsec:challenges}
Trivially embedding a \ac{dnn} is unrealistic due to the main challenges of realizing such an extension below.
%In contrast, offloading the computation process of \ac{dnn} into the network can effectively free up the computation resources on the server side.
%Offloading the inference process of a \ac{dnn} to the network requires splitting the \ac{dnn} model into multiple neuron blocks to be distributed and deployed on the network nodes.
\begin{enumerate}
    \item \emph{Resource-constrained \ac{upf}}: \ac{dl} is computationally demanding, and it often requires a complex computing architecture (such as dedicated hardware like GPU and large memory). Although future \ac{upf} element will be programmable with compute-oriented resources onboard, its computational power is way much less than a \ac{cots} server node. Nevertheless, the size of a \ac{dnn} is usually huge ~\cite{Zhang2019DeepLearningMobile}. Hence, a central question is how to split a \ac{dnn} into pieces that are network element-suitable;
    \item \emph{Limited number of network nodes}: \xxcmt{Not quite sure about this challenge. More \acp{upf} will be better? If so, unfortunately, in a mobile network, I am quite sure that the \ac{upf}$\sharp$  is often just $2$-$5$. I think you should say inter-layer data explosion is the 2nd challenge.} In a local network, packet is usually forwarded through a few or a dozen network nodes. In a public network, the maximum number of intermediate nodes is a few hundred, occasionally more than 1000. However, today's \ac{dnn}s have evolved into large scale neuronal clusters, where the number of neurons can easily reach thousands or even more, e.g., ***\hwcmt{For JH: giving some examples?}. As a result, a brute-force approach to the distributed deployment of \ac{dnn}s in neurons would limit the offload potential significantly.
\end{enumerate}

% Due to the massive parameters of \ac{dnn}s, it usually needs to occupy the main computational resources on the server-side.
% And offloading the \ac{dnn} computation process to the network can effectively free up the computational resources on the server-side.
% In practical deployment and inference, most \ac{dnn}s use a straightforward computational structure, i.e., each neural network layer needs to be computed only once.
% Intuitively, offloading computational processes to the network requires splitting and deploying different parts of the NN model in different VNFs.
% However, the following challenges usually need to be addressed to accomplish this goal.
% \begin{enumerate}
%     \item Limited computing resources: Typically, VNF devices have limited computing resources. It cannot run all the computational processes like the server side.
%     Therefore, when deploying computational processes in VNF, it is necessary to consider whether the deployed computational processes and resources match. Also, when there are multiple VNFs, the computing resources of each VNF should be utilized as evenly as possible.
%     \item Additional cache time: When a deep learning model performs inference, the computational process of most layers requires the entire output of the previous layer as input.
%     Compared to centralized deployments, VNFs require additional storage time to receive the data required for computation.
%     Therefore, the deployment needs to be designed in a way to offset the impact of the extra storage time on the service latency.
% \end{enumerate}

\subsubsection{Design principles}
%\hwcmt{1. smash strategy. 2. glue strategy. 3. fusion strategy.}

%\xxcmt{It's confusing with the three strategies above and the three principles below. Which is exactly your principle and which other is your strategies?}



%In practical deployment and inference, each neural network layer of a \ac{dnn} is computed only once in most \ac{dnn}s.

%To satisfy the three principles proposed above, we divide the model in the following way.
Considering the challenges above, we propose the following principles when a \ac{nn} model needs to be split.
\begin{enumerate}
    \item \emph{Evenly splitting a model:} Splitting the model into even sizes can improve \ac{upf} resource utilization.\xxcmt{I think it be proportional to \ac{upf}'s resource availability.}
    \item \emph{\xxtext{Avoiding inter-\ac{upf} traffic explosion}:} \xxcmt{Then, here it nicely matches to the 2nd challenge before to say another principle is to avoid such an explosion.} A \ac{dnn} transforms raw data into high-dimensional feature representations by convolution or other operations. This process is usually accompanied by a variation in the scale of the data. To ensure that the transmission time after splitting is minimized, it is usually necessary to analyze the data traffic when splitting the model and split it in the locally optimal part if possible. \xxtext{Achieving this objective often contradicts to the first one, therefore, a joint consideration is needed}.
    \item \xxtext{\emph{Parallelizing local processing and forwarding}: Local \ac{dl} on a \ac{upf} requires data and temporal outputs of the last layer of a \ac{nn} delivered from the previous \ac{upf}. Caching and waiting the required inputs take time, especially when the path length increases. Hence, parallelizing the underlying forwarding strategy and efficient inter-\acp{upf} interactions should be considered.}    
%    For VNFs with deployed sub-models, at computation time, each VNF is required to wait for all the computation results of the previous VNF, called cache time. As the number of VNFs increases, the storage time naturally increases. To reduce this additional time overhead, it is necessary to parallelize computation and transmission when deploying and transmitting data, i.e., perform computation while transmitting data that is unrelated to this VNF computation.
\end{enumerate}
%\xxcmt{After I stopped here, I realized the above three bullets are your principles.}
\xxtext{Bearing the three principles above, a generic way to realize the DP \ac{dl} capability extension can follow the procedures below:}
first, to ensure that the computational resources of each VNF can be fully utilized, the number of parameters and computational complexity of the model's different layers need to be analyzed.\xxcmt{the text above still reads like guidelines. Here, directly introduce what has to be done so that the three principles can be covered/fulfilled.} \xxcmt{You should say: ``the first step is to ...''; ``the second step is to ...''; ``the third step is to ...'' After the steps, the DP DL enhancement should be achieved.} It is guaranteed that the sub-models do not exceed the computational capacity limitation of the VNF after deployment.
Second, when considering the division place, it is necessary to analyze the data flow and the scale of the data in different parts of the model.
Normally, the data flow direction of the model is straightforward.
Therefore, only a single-link network structure needs to be considered when setting up the VNF.


\subsection{Management and control plane extension}
The DP enhancement alone does not finish a complete enhancement of 6G system due to lack of management and control plane operational procedures. There are two additional extensions that have to be done, which are: management and control planes.

\subsubsection{Management plane extension}
\xxcmt{TBD...}




\subsubsection{Control plane extension}
\xxcmt{TBD...}



In summary, DP and M-/CP enhancements introduced above together complete the picture of enhancing in-network \ac{dl} capability for \ac{ml} inference application services in 6G.

==> sections/backup_xunxiao/introduction.tex <==
\section{Introduction}\label{sec:introduction}



\xxcmt{I searched some papers and try to purify our idea. There are some work about using NN to do inference for sure (e.g., do classification and so on). Therefore, we cannot just claim that ours is about cutting NNs into network devices and study its challenges.}

\xxcmt{We should go one level down, to say: we study BSS problem solved with NNs with COIN concept. Under this line, we clarify: 1. why BSS problem is different from other types of problems that are solved with using NNs, in order to show the uniqueness of our studied problem; 2. How BSS problem is solved with NNs in the literature, what are considered and what are not, to show our novelty and contributions; 3. For those not considered challenges/problems/potential issues, what's our opinions> why they are important. With this general logic flow, I think the whole idea should hold.}

\xxcmt{With the SotA, then in the following sections, we can start to introduce the method cutting NNs into networks with well justifications. After that, we start to introduce its opponent--pICA. Once this is done, we can go into the evaluation settings and results. At the end, we should put extensive and intensive discussions on the yielded observations; then we give our takeaway messages.}

AI in 6G and its impact on the design of open programmable networks in the next-generation wireless networks




\xxcmt{Only 15 references are allowed? I included the following papers:} \cite{Sapio2017NetworkComputationisa,Sanvito2018Cannetworkbe,Zhang2019DeepLearningMobile,Dutta2020DiscrepancyTheoreticalAnalysis,XiangOpenSourceTestbed,Liang2020edgebaseddeep,Xu2021GRACECompressedCommunication,Xavier2021ProgrammableSwitchesNetworking,Wu2021AbstractionbasedMulti,Wu2021NetworkProcessingAcoustic,Saquetti2021NetworkIntelligenceRunning,Wu2021ComputingMeetsNetwork,Yuan2022UnlockingPowerInline}

\hwcmt{Currently, the number of references is more than 15, we will remove some of them after all text is fixed.}

==> sections/backup_xunxiao/method.tex <==
\section{Method}\label{sec:method}
\subsection{Introduction of Conv-TasNet}
Conv-TasNet is an end-to-end time-domain speech separation method based on convolutional neural networks (CNN).
In Conv-TasNet,  the mixed mono waveform is patterned with a fully convolutional encoder-decoder model, which consists of three main components, namely encoder, separation, and decoder.

Encoder, as a collection of filters, maps the input time-domain signal data into a high-dimensional feature space $E$.
Meanwhile, this part of the data is reconstructed in the decoder to derive the separated signal, as shown in \cref{fig:conv_tasnet_arch}.

The separation part, as the main part of the model parameters, occupies most of the computational resources.
Its role is to extract the mask $M$ corresponding to each source to be separated from the encoder output $E$.
It is a stack of several 1D convolutional blocks with the same structure.
At the end of the separation process, an individual 1D-convolutional layer is attached to generate the mask according to the number of sources.

The decoder is designed to restore each individual source.
In the decoder operation, the high-dimensional feature data corresponding to each source is first obtained by the dot product of mask $M $and encoder data $E$.
After that, a 1D deconvolution layer is simply used to map the data from the feature space back to the time domain.
\begin{figure*}[t]
	\centerline{\includegraphics[width=\textwidth]{figures/conv-tasnet_new.pdf}}
	\caption{The architecture of Conv-TasNet and the corresponding network settings. Depending on the number of VNFs, the computational process is offloaded into the vnf network in different ways. Data transfer and computation are processed in parallel as much as possible, and data generated by the encoder is forwarded to the server in parallel while VNFs are computing to reduce service latency. In the figure, the green part represents the data generated by the encoder (VNF1 according to our setting), and the red part the data generated during the calculation of other VNFs. The data generated by the encoder is directly transmitted to the server-side. The server-side can receive the encoder data before receiving the VNF data. \hwcmt{The deployment method and time analysis could be divided into two figures, which are described and discussed separately.}}
	\label{fig:conv_tasnet_arch}
\end{figure*}



\subsection{Challenges}\label{subsec:challenges}
Due to the massive parameters of deep neural networks, it usually needs to occupy the main computational resources on the server-side.
And offloading the deep neural network computation process to the network can effectively free up the computational resources on the server-side.
In practical deployment and inference, most deep neural networks use a straightforward computational structure, i.e., each neural network layer needs to be computed only once.
Intuitively, offloading computational processes to the network requires splitting and deploying different parts of the NN model in different VNFs.
However, the following challenges usually need to be addressed to accomplish this goal.
\begin{enumerate}
	\item Average arithmetic power: To maximize the use of the network's VNF devices, it is often necessary to split the model as evenly as possible.
	\item Local optimal data traffic: Deep neural networks transform raw data into high-dimensional feature representations by convolution or other operations. This process is usually accompanied by a variation in the scale of the data. To ensure that the transmission time after splitting is minimized, it is usually necessary to analyze the data traffic when splitting the model and split it in the locally optimal part if possible. This process sometimes conflicts with the first principle and requires appropriate trade-offs.
	\item Parallelization of computation and transmission: For VNFs with deployed sub-models, at computation time, each VNF is required to wait for all the computation results of the previous VNF, called cache time. As the number of VNFs increases, the storage time naturally increases. To reduce this additional time overhead, it is necessary to parallelize computation and transmission when deploying and transmitting data, i.e., perform computation while transmitting data that is unrelated to this VNF computation.
\end{enumerate}

\subsection{Deployment}
To satisfy the three principles proposed above, we divide the model in the following way.
For a generic neural network model, the following analysis process is required to be performed when offloading to the network.

First, to ensure that the computational resources of each VNF can be fully utilized, the number of parameters and computational complexity of the model's different layers need to be analyzed. It is guaranteed that the sub-models do not exceed the computational capacity limitation of the VNF after deployment.
Second, when considering the division place, it is necessary to analyze the data flow and the scale of the data in different parts of the model.
Normally, the data flow direction of the model is straightforward.
Therefore, only a single-link network structure needs to be considered when setting up the VNF.


Following the instructions of Conv-TasNet, we set up four blocks in the separation section, which have fixed sizes of input and output and the output data volume is relatively minimal.
Meanwhile, the encoder is always placed in the first vnf to receive the raw data, and the decoder is always deployed in the server to get the final result.
Since the final convolutional layer in the separation part exponentially scales up the data volume depending on the number of sources.
To save service latency it is merged with the decoder into one part.

\hwcmt{Generalising the description of deployments, rather than limiting it to specific 1, 3, and 5 VNFs.}
When the number of VNFs grows, it represents a gradual enrichment of computing resources within the network.
In order to simulate the deployment characteristics of the model with different computing resources, we set three cases with $VNF=1,3,5$.\xxcmt{I think the following three bullets are not necessary.}

\begin{enumerate}
    \item $VNF=1$: In this case, the separation part cannot be fully deployed in the VNF considering the limited network computing resources.
    Therefore, we evenly split the model and deploy the encoder and the first two blocks of the separation part in the unique VNF.
    In order to ensure the parallelization of computation and transmission, the data $E$ obtained after encoder computation is sent directly to the server-side, while the VNF continues to compute the mask data $M$ using $E$.
    On the server side, when the collection of the mask data $M$ is finished, the collected data is forwarded to the other two separate modules to derive the final mask $M$.
    \item $VNF=3$: In this setup, there are enough computing resources to allocate all the separation blocks.
    We deploy the four blocks equally in the last two VNFs while the encoder is deployed in the first VNF and the decoder is deployed on the server.
   The output $E$ from the encoder is sent to the second VNF, but also directly to the server.
   After receiving $E$ from VNF1 and $M$ from the last VNF, the server-side can directly calculate the final separation result.
   \item $VNF=5$: Similar to the case of VNF=3, the four blocks are equally allocated to the four VNFs.
\end{enumerate}

It is worth noting that as the number of VNFs increases, the distribution of models becomes increasingly "sparse".
Since the results of each layer of the neural network must use all the data of the previous layer, it leads to a gradual increase in the cache time of each VNF.

\subsection{AI as network functions}
